A Survey on Visual Anomaly Detection: Challenge, Approach, and Prospect

Visual Anomaly Detection (VAD) endeavors to pinpoint deviations from the concept of normality in visual data, widely applied across diverse domains, e.g., industrial defect inspection, and medical lesion detection. This survey comprehensively examines recent advancements in VAD by identifying three primary challenges: 1) scarcity of training data, 2) diversity of visual modalities, and 3) complexity of hierarchical anomalies. Starting with a brief overview of the VAD background and its generic concept definitions, we progressively categorize, emphasize, and discuss the latest VAD progress from the perspective of sample number, data modality, and anomaly hierarchy. Through an in-depth analysis of the VAD field, we finally summarize future developments for VAD and conclude the key findings and contributions of this survey.

==> figures/fig_vision_data.tex <==
\begin{figure}[t]
\centering\includegraphics[width=\linewidth]{figures/concept_illustration.pdf}
\caption{\textbf{Concept of composition process for vision data and anomalies.} Each image frame $v \in \mathcal{V}$ is formed by combining multiple entities $\mathcal{X}$ through individual relationship functions $\varphi$ $\in$ $\Phi$. For the image frames $\mathcal{V}$, we illustrate normal frames, frames with structural anomalies, and frames with semantic anomalies.}%\vspace{-5mm}
\label{fig:semantic-ad}
\end{figure}

==> figures/table_performance.tex <==

% \begin{table*}[t]
% \begin{minipage}[t]{\linewidth}
%     \centering
%      \resizebox{\linewidth}{!}{%
%     \input{figures/table_performance_sample_number}
%     }
%     \caption{Sample Number Table}
% \end{minipage}

% \begin{minipage}[t]{0.5\linewidth}
%   \centering
%   \resizebox{\linewidth}{!}{%
%   \input{figures/table_performance_modality}
%   }
%   \caption{Modality Table}
% \end{minipage}%
% \begin{minipage}[t]{0.5\linewidth}
%   \centering
%   \resizebox{\linewidth}{!}{%
%   \input{figures/table_performance_hierarchy}
%   }
%   \caption{Hierarchy Table}
% \end{minipage}

%   % \begin{minipage}{1\textwidth}
%   %   \centering
%   %   \input{figures/table_performance_sample_number}
%   %   \caption{Sample Number Table}
%   % \end{minipage}%
%   % \begin{minipage}{0.5\textwidth}
%   %   \centering
%   %   \begin{minipage}{0.5\textwidth}
%   %     \centering
%   %     \input{figures/table_performance_modality}
%   %     \caption{Modality Table}
%   %   \end{minipage}%
%   %   \begin{minipage}{0.5\textwidth}
%   %     \centering
%   %     \input{figures/table_performance_hierarchy}
%   %     \caption{Hierarchy Table}
%   %   \end{minipage}
%   % \end{minipage}
% \end{table*}

% % \input{figures/table_performance_sample_number}
% % \input{figures/table_performance_modality}
% % \input{figures/table_performance_hierarchy}

